End-to-End Time-Lapse Video Synthesis from a Single Outdoor Image

Time-lapse videos usually contain visually appealing content but are often difficult and costly to create. In this paper, we present an end-to-end solution to synthesize a time-lapse video from a single outdoor image using deep neural networks. Our key idea is to train a conditional generative adversarial network based on existing datasets of time-lapse videos and image sequences. We propose a multi-frame joint conditional generation framework to effectively learn the correlation between the illumination change of an outdoor scene and the time of the day. We further present a multi-domain training scheme for robust training of our generative models from two datasets with different distributions and missing timestamp labels. Compared to alternative time-lapse video synthesis algorithms, our method uses the timestamp as the control variable and does not require a reference video to guide the synthesis of the final output. We conduct ablation studies to validate our algorithm and compare with state-of-the-art techniques both qualitatively and quantitatively.

==> figures/fig_multidomain_failure.tex <==
\begin{figure}[t]
\begin{center}
\begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=0.31\linewidth]{multi_domain/0/original.png}
    \includegraphics[width=0.31\linewidth]{multi_domain/0/071200.png}
    \includegraphics[width=0.31\linewidth]{multi_domain/0/071200_t.png}

    \includegraphics[width=0.31\linewidth]{multi_domain/1/original.png}
    \includegraphics[width=0.31\linewidth]{multi_domain/1/163335.png}
    \includegraphics[width=0.31\linewidth]{multi_domain/1/163335_t.png}
    \caption{Before and after $\generatoramos$}
\end{subfigure}

\begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=0.31\linewidth]{failure_cases/0/original.png}
    \includegraphics[width=0.31\linewidth]{failure_cases/0/out_114536.png}

    \includegraphics[width=0.31\linewidth]{failure_cases/1/original.png}
    \includegraphics[width=0.31\linewidth]{failure_cases/1/out_192624.png}
    \caption{Failure cases}
\end{subfigure}
\end{center}
\caption{Some examples of before and after $\generatoramos$ (a), and failure cases (b). In (a), each image from left indicates the input, the output of $\generatortlvdb$, and the output of $\generatoramos$, respectively. In (b), the left image is the input, and the right image is the output.
% \snam{Or 4-5 different scenes?}
% \chongyang{(11/11/2018) Please explain each column/row. It is always to good to prepare more scenes so that we can choose the best ones for the final submission.}
% \snam{What I meant is adding 5 different input images on the top and their corresponding translated images on the bottom. But, it is not consistent with arrangement in other figures.}
% \chongyang{(11/12/2018) Somehow I feel this figure is not very intuitive to understand. My concern is that the changes before and after $\generatoramos$ are inconsistent across the four frames. But I don't have a strong opinion here.}
\snam{I put two figures here together because both figures do not need much space. Separating them may be waste of space.}
}
\label{fig:multidomain_failure}
\end{figure}


==> figures/fig_result_gallery.tex <==
\newcommand\galleryfigurewidth{0.16}
\begin{figure*}[t]
\begin{center}
 \centering
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/0/original.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/0/out_152847.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/0/out_170935.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/0/out_182847.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/0/out_185736.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/0/out_193335.png}
 
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/1/original.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/1/out_065735.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/1/out_070447.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/1/out_071912.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/1/out_085248.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/1/out_104047.png}
 
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/2/original.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/2/out_145248.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/2/out_164047.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/2/out_175248.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/2/out_185736.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/2/out_190448.png}
 
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/3/original.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/3/out_160448.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/3/out_174536.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/3/out_182135.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/3/out_182847.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/3/out_183559.png}
 
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/4/original.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/4/out_074047.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/4/out_074759.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/4/out_075512.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/4/out_080936.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/4/out_100447.png}
 
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/5/original.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/5/out_062848.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/5/out_071200.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/5/out_071912.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/5/out_074047.png}
 \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery_v2/5/out_085248.png}
 
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/0/original.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/0/out_073335.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/0/out_074759.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/0/out_082359.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/0/out_120000.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/0/out_183559.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/0/out_185736.png}
 
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/1/original.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/1/out_074047.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/1/out_082359.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/1/out_124311.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/1/out_173112.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/1/out_183559.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/1/out_190448.png}
 
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/2/original.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/2/out_071200.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/2/out_073335.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/2/out_120000.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/2/out_173112.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/2/out_193335.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/2/out_195511.png}
 
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/3/original.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/3/out_060000.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/3/out_071200.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/3/out_120000.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/3/out_172400.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/3/out_190448.png}
%  \includegraphics[width=\galleryfigurewidth\linewidth]{result_gallery/3/out_194047.png}
\end{center}
\caption{Our prediction results of the input images at different times of a day. The input images are shown on the left in each row.
%\chongyang{(10/07/2018) 1. Save each individual image as separate file with the timelapse as part of the file name; 2. The temporal sampling rate is a bit too high (maybe half of the images for each input will be enough).} 
%\menglei{(11/07/2018) I like these results! But the second column of the first row might be too dark.}
%\ning{(10/15/2018) I think probably 4-6 representative images for each input would be good enough.}
%\chongyang{(10/23/2018) Let's prepare more than 10 output frames for each input image just in case we may need more later.}
% \snam{I'm going to add some results here. But, I'm worried about symmetric change of color tone. If color tone of sunrise and sunset is similar, is it still convincing?}
% \chongyang{(11/07/2018) I have two suggestions: (1) if possible, try to avoid very similar output images for the same input; (2) as I also commented under Figure~\ref{fig:teaser}, maybe we can reorder the sequence based on the overall brightness for more intuitive visualization instead of timestamps, assuming we are not going to show the timestamps anyway.}
%\snam{Can we insert a reference frame to each baseline image? e.g. small box in a baseline image. In addition, can we insert a blank image in the first row?}
%\chongyang{(11/10/2018) Hmm, this new version looks quite confusing to me. From the file paths, it seems to be about comparisons against~\cite{Li:2018:LII} and \cite{Shih:2013:DHD}. Then these comparisons should be put into another figure (\Fref{fig:comparisons}), rather than replacing our gallery. The vertical arrangement for the time of a day is a bit counter-intuitive and not consistent with other figures in our paper. Also, why only three output frames for each method? Can we have something like \Fref{fig:ablation_study}?}
%\snam{I moved the comparison to \fref{fig:comparisons}. But, I'm still not satisfied with our current visualization. I'm considering putting original videos here if I can find something good to show.}
\snam{Let's choose three or four best results. I think it would be good if at least one of our results contains night scene. But, if the quality is bad, I'm willing to remove it.}
}
\label{fig:result_gallery}
\end{figure*}


==> final.tex <==
% \newcommand{\final}{1}
\input{main}

